T-Net: Deep Stacked Scale-Iteration Network for Image Dehazing

Hazy images reduce the visibility of the image content, and haze will lead to failure in handling subsequent computer vision tasks. In this paper, we address the problem of image dehazing by proposing a dehazing network named T-Net, which consists of a backbone network based on the U-Net architecture and a dual attention module. And it can achieve multi-scale feature fusion by using skip connections with a new fusion strategy. Furthermore, by repeatedly unfolding the plain T-Net, Stack T-Net is proposed to take advantage of the dependence of deep features across stages via a recursive strategy. In order to reduce network parameters, the intra-stage recursive computation of ResNet is adopted in our Stack T-Net. And we take both the stage-wise result and the original hazy image as input to each T-Net and finally output the prediction of clean image. Experimental results on both synthetic and real-world images demonstrate that our plain T-Net and the advanced Stack T-Net perform favorably against the state-of-the-art dehazing algorithms, and show that our Stack T-Net could further improve the dehazing effect, demonstrating the effectiveness of the recursive strategy.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> name.tex <==
%% 表1
\begin{table*}[htbp]
\centering
\caption{Comparison on the SOTS dataset for T-Net with different configurations.}
\begin{tabular}{Ic|c|c|c|c|c|c|cI}
\Xhline{0.8pt}
\multicolumn{2}{Ic|}{Configuration} & \multicolumn{2}{c|}{Indoor} & \multicolumn{2}{c|}{Outdoor}  & \multicolumn{2}{cI}{SOTS (In \& Out)}\\
\Xhline{0.8pt}
\multicolumn{1}{IC{1.2cm}|}{m} &\multicolumn{1}{C{1.2cm}|}{n} & \multicolumn{1}{C{1.2cm}|}{PSNR} & \multicolumn{1}{C{1.2cm}|}{SSIM} & \multicolumn{1}{C{1.2cm}|}{PSNR} & \multicolumn{1}{C{1.2cm}|}{SSIM} & \multicolumn{1}{C{1.2cm}|}{PSNR} & \multicolumn{1}{C{1.2cm}I}{SSIM} \\
\Xhline{0.8pt}
\multirow{2}[3]{*}{3} & 2     &21.55 &0.8622 &24.25 &0.9286 &22.90 &0.8954 \\
\cline{2-8}           & 4     &25.29 &0.9313 &28.44 &0.9588 &26.86 &0.9451 \\ 
\cline{2-8}           & 6     &26.56 &0.9385 &28.29 &0.9560 &27.43 &0.9473 \\ 
\hline
\multirow{2}[3]{*}{4} & 2     &21.76 &0.8631 &24.19 &0.9267 &22.97 &0.8949 \\ 
\cline{2-8}           & 4     &26.94 &0.9444 &28.04 &0.9596 &27.49 &0.9520 \\ 
\cline{2-8}           & 6     &26.93 &0.9436 &29.34 &0.9635 &28.13 &0.9536 \\ 
\hline
\multirow{2}[3]{*}{5} & 2     &21.86 &0.8620 &23.86 &0.9244 &22.86 &0.8932\\ 
\cline{2-8}           & 4     &27.32 &0.9447 &29.28 &0.9624 &28.30 &0.9535\\ 
\cline{2-8}           & 6     &27.74 &0.9458 &29.35 &0.9628 &\textbf{28.55} &\textbf{0.9543}\\ 
\Xhline{0.8pt}
\end{tabular}%
\end{table*}%
%表二
\begin{table*}[htbp]
\centering
\caption{Comparison on the SOTS dataset for several variants of T-Net.}
\begin{tabular}{Ip{5.5cm}|c|c|c|c|c|cI}
\Xhline{0.8pt}
\multicolumn{1}{Ic|}{\multirow{1}[4]{*}{Variant}} & 
\multicolumn{2}{c|}{Indoor} & \multicolumn{2}{c|}{Outdoor} & \multicolumn{2}{cI}{SOTS (In \& Out)} \\
\cline{2-7}          & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{cI}{SSIM} \\
\Xhline{0.8pt}
the basic model                         &24.59 &0.8537 &23.78 &0.7920 &24.19 &0.8228\\ 
\hline
with usual skip connections (1x1 conv)  &26.88 &0.9413 &27.96 &0.9594 &27.42 &0.9504\\ 
\hline
with usual skip connections (RDB block) &26.95 &0.9441 &28.27 &0.9598 &27.61 &0.9520\\ 
\hline
with our skip connections               &27.36 &0.9454 &28.28 &0.9606 &27.82 &0.9530\\ 
\hline
T-Net                       &27.74 &0.9458 &29.35 &0.9628 &\textbf{28.55} &\textbf{0.9543}\\
\Xhline{0.8pt}
\end{tabular}%
\end{table*}%
%表三
\begin{table*}[htbp]
\centering
\caption{Comparison on the SOTS dataset for Stack T-Net with different $K$ stages.}
\begin{tabular}{Ic|c|c|c|c|c|cI}
\Xhline{0.8pt}
\multirow{1}[4]{*}{Recursive stage number} & \multicolumn{2}{c|}{Indoor} & \multicolumn{2}{c|}{Outdoor} & \multicolumn{2}{cI}{SOTS (In \& Out)}\\
\cline{2-7}          & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{c|}{SSIM} & \multicolumn{1}{c|}{PSNR} & \multicolumn{1}{cI}{SSIM}\\
\Xhline{0.8pt}
$K=1$   &27.74 &0.9458 &29.35 &0.9628 &28.55 &0.9543 \\ 
\hline
$K=2$   &27.58 &0.9463 &29.85 &0.9650 &28.71 &0.9556 \\ 
\hline
$K=3$   &27.73 &0.9453 &29.93 &0.9649 &28.83 &0.9551 \\ 
\Xhline{0.8pt}
\end{tabular}%
\end{table*}%
%% 表四
\begin{table}[htbp]
\centering
\caption{Quantitative comparison on SOTS dataset for the state-of-the-art dehazing methods.}
\begin{tabular}{IC{2.4cm}|C{1.0cm}|C{1.0cm}I}
\Xhline{0.8pt}
\multirow{1}[4]{*}{Methods} & \multicolumn{2}{cI}{SOTS} \\
\cline{2-3}          & PSNR  & SSIM\\
\Xhline{0.8pt}
DCP \cite{5567108}   & 15.49  & 0.64 \\
\hline
NLD \cite{Berman_2016_CVPR}  & 17.27 & 0.75 \\
\hline
MSCNN \cite{2016Single} & 17.57 & 0.81 \\
\hline
DehazeNet \cite{2016DehazeNet} & 21.14 & 0.85 \\
\hline
AOD-Net \cite{8237773} & 19.06 & 0.85 \\
\hline
DCPDN \cite{8578435} & 19.39 & 0.65 \\
\hline
GFN \cite{Ren_2018_CVPR}  & 22.30 & 0.88  \\
\hline
EPDN \cite{8953692} & 23.82 & 0.89 \\
\hline
DA\_dehazing \cite{Shao_2020_CVPR} & 27.76 & 0.93 \\
\hline
T-Net & 28.55 & 0.95  \\
\hline
Stack T-Net &28.83 &0.96  \\
\Xhline{0.8pt}
\end{tabular}%
\end{table}%
